One of Many: Assessing User-level Effects of Moderation Interventions on r/The_Donald

Evaluating the effects of moderation interventions is a task of paramount importance, as it allows assessing the success of content moderation processes. So far, intervention effects have been almost solely evaluated at the aggregated platform or community levels. Here, we carry out a multidimensional evaluation of the user-level effects of the sequence of moderation interventions that targeted r/The_Donald: a community of Donald Trump adherents on Reddit. We demonstrate that the interventions: 1) strongly reduced user activity; 2) slightly increased the diversity of the subreddits in which users participated; 3) slightly reduced user toxicity; and 4) gave way to the sharing of less factual and more politically biased news. Importantly, we also find that interventions having strong community level effects are associated to extreme and diversified user-level reactions. Our results highlight that community-level effects are not always representative of the underlying behavior of individuals or smaller user groups. We conclude by discussing the practical and ethical implications of our results. Overall, our findings can inform the development of targeted moderation interventions and provide useful guidance for policing online platforms.

==> ethics.tex <==
\section{Ethics Statement}
\label{sec:ethics}
We strongly believe that this work will have a positive broader impact on the policing of online platforms by providing novel and valuable findings for informing future content moderation decisions. Part of our results showed that certain moderation interventions can radicalize a minority of the moderated users. We discussed the ethical implications of these results, including the need to carefully balance the risk of causing harms to minorities in pursuit of benefits for the larger community.

This work is entirely based on public Reddit data, which was enriched with indicators of toxicity, and of the political bias and factuality of linked news articles.
Given the sensitive information about user activities, the main ethical risk of this work is the potential deanonymization of the dataset. We mitigated this risk by pseudonymization. In addition, we remark that the base dataset that we used fully abides by the FAIR principles, since it is published in an interoperable and machine-readable format, and under a reusable license. Further, it is indexed on the reference platform Zenodo, with an associated DOI.

